Forever Young: Aging Control For Smartphones In Hybrid Networks

The demand for Internet services that require frequent updates through small messages, such as microblogging, has tremendously grown in the past few years. Although the use of such applications by domestic users is usually free, their access from mobile devices is subject to fees and consumes energy from limited batteries. If a user activates his mobile device and is in range of a service provider, a content update is received at the expense of monetary and energy costs. Thus, users face a tradeoff between such costs and their messages aging. The goal of this paper is to show how to cope with such a tradeoff, by devising \emph{aging control policies}. An aging control policy consists of deciding, based on the current utility of the last message received, whether to activate the mobile device, and if so, which technology to use (WiFi or 3G). We present a model that yields the optimal aging control policy. Our model is based on a Markov Decision Process in which states correspond to message ages. Using our model, we show the existence of an optimal strategy in the class of threshold strategies, wherein users activate their mobile devices if the age of their messages surpasses a given threshold and remain inactive otherwise. We then consider strategic content providers (publishers) that offer \emph{bonus packages} to users, so as to incent them to download updates of advertisement campaigns. We provide simple algorithms for publishers to determine optimal bonus levels, leveraging the fact that users adopt their optimal aging control strategies. The accuracy of our model is validated against traces from the UMass DieselNet bus network.

==> proofj.tex <==
\subsection{Proof of Proposition~\ref{blabla}}
\begin{proof}
The increase (or decrease) of the bonus level $B$ is equivalent to the decrease (or increase) of price $P_W$.
According to Proposition \ref{increasing}, the optimal threshold $s^{\star}$ is
a non-increasing function of $B$.

To prove this proposition, we first show that the average age is reduced when the threshold $s$ decreases.
Consider two threshold policies $s$ and $s+1$. Let $Age_1$ and $Age_2$ be their average ages. We obtain
\begin{eqnarray*}
Age_1 &=& \sum_{i=1}^{s}\frac{i}{s+\frac{1-p}{p}} + \sum_{i=s+1}^{M-1}\frac{i\cdot (1-p)^{i-s}}{s+\frac{1-p}{p}} \nonumber\\
&& + \frac{(1-p)^{M-s}}{p}\cdot \frac{M}{s+\frac{1-p}{p}}; \\
Age_2 &=& \sum_{i=1}^{s+1}\frac{i}{s+1+\frac{1-p}{p}} + \sum_{i=s+2}^{M-1}\frac{i\cdot (1-p)^{i-s-1}}{s+1+\frac{1-p}{p}} \nonumber\\
&& + \frac{(1-p)^{M-s-1}}{p}\cdot \frac{M}{s+1+\frac{1-p}{p}}.
\end{eqnarray*}
Therefore, by using some transformations, we have
\begin{eqnarray}
&& Age_1 \cdot \frac{s+\frac{1-p}{p}}{s+1+\frac{1-p}{p}} = \sum_{i=1}^{s}\frac{i}{s+1+\frac{1-p}{p}} \nonumber\\
&& + \sum_{i=s+1}^{M-1}\frac{i\cdot (1-p)^{i-s}}{s+1+\frac{1-p}{p}} + \frac{(1-p)^{M-s}}{p}\cdot \frac{M}{s+1+\frac{1-p}{p}};\\
&& Age_2 \cdot (1-p) = \sum_{i=1}^{s+1}\frac{i(1-p)}{s+1+\frac{1-p}{p}} \nonumber\\
&& + \sum_{i=s+2}^{M-1}\frac{i\cdot (1-p)^{i-s}}{s+1+\frac{1-p}{p}} + \frac{(1-p)^{M-s}}{p}\cdot \frac{M}{s+1+\frac{1-p}{p}}.
\end{eqnarray}
We subtract the left-hand of above expressions and obtain
\begin{eqnarray}
&& Age_1 \cdot \frac{s+\frac{1-p}{p}}{s+1+\frac{1-p}{p}}  - Age_2 \cdot (1-p) \nonumber\\
&& = Age_1-Age_2 -Age_1\cdot\frac{1}{s+1+\frac{1-p}{p}} + Age_2\cdot p \nonumber\\
&& = (Age_1 -Age_2)(1-p) + Age_1\cdot \frac{ps}{s+1+\frac{1-p}{p}}.
\end{eqnarray}
We then subtract the right-hand of the above expressions,
\begin{eqnarray}
\textrm{righthand} \;\; = \sum_{i=1}^{s}\frac{pi}{s+1+\frac{1-p}{p}}.
\end{eqnarray}
Combining the right-hand and left-hand equations together, we have
\begin{eqnarray}
(Age_1 -Age_2)(1-p) = \frac{p}{s+1+\frac{1-p}{p}}\big( \sum_{i=1}^{s}i - s\cdot Age_1 \big).
\end{eqnarray}
The average of the threshold policy $s$ is a function of the probability $p$. The smallest
average age is obtained when $p$ is 0 (i.e. the system is periodic). The average age
at $p=0$ is expressed as
\begin{eqnarray}
Age_1^{\min} = \frac{1}{s}\sum_{i=1}^{s}i.
\end{eqnarray}
Therefore, one can see that the following inequality holds
\begin{eqnarray}
Age_1 < Age_2.
\end{eqnarray}
We can conclude that for any two threshold policies $s_1$ and $s_1$ that has $s_1<s_2$, the average
ages satisfy
\begin{eqnarray}
Age_{s_1} < Age_{s_2}.
\end{eqnarray}
Let us go back to the bonus level. The optimal threshold $s$ is a one-to-one mapping of $B$. However, the
inverse function does not exist because it is not a one-to-one mapping. Here, we denote $\underline{B}_s$
and $\overline{B}_s$ be the lower and upper bonus levels for the optimal threshold $s$.
We analyze two cases on how the publisher chooses the bonus $B$ so as to minimize the average age.

i). If $s(P_W) < \frac{Np}{T}-\frac{1-p}{p}$, then the constraint in Eq.(\ref{}) cannot be satisfied
with the highest allowable bonus. To minimize the average age, the feasible bonus $B$ can be chosen
from the range $[\underline{B}_{s(P_W)}, P_W]$.

ii). If $s(P_W) > \frac{Np}{T}-\frac{1-p}{p}$, there is a unique optimal threshold $s^{\star}$.
We explain the reason as below.
The objective function in Eq.(\ref{}) is an increasing function of the threshold policy $s$,
while the constraint in Eq.(\ref{}) is a decreasing function of $s$. Therefore, the optimal
threshold policy to minimize the average age is given by
\begin{eqnarray}
s^{\star} = \min(M+1, [\frac{Np}{T}-\frac{1-p}{p}]^{+}).
\end{eqnarray}
The corresponding bonus level $B$ can be chosen from the range $[\underline{B}_{s^{\star}}, \overline{B}_{s^{\star}}]$.

\end{proof}
